Efficient semantic image segmentation with superpixel pooling

In this work, we evaluate the use of superpixel pooling layers in deep network architectures for semantic segmentation. Superpixel pooling is a flexible and efficient replacement for other pooling strategies that incorporates spatial prior information. We propose a simple and efficient GPU-implementation of the layer and explore several designs for the integration of the layer into existing network architectures. We provide experimental results on the IBSR and Cityscapes dataset, demonstrating that superpixel pooling can be leveraged to consistently increase network accuracy with minimal computational overhead. Source code is available at https://github.com/bermanmaxim/superpixPool

==> blockspix_orig.tex <==
\begin{table}[h]\small
\centering
\caption{Dice coefficients of the V3 networks using different shapes and sizes of superpixels.}
\label{tab:comparison}
\begin{tabular}{lllll}
\topline
               & Baseline & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}BLOCK (V3)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SLIC (V3)\end{tabular}} \\ \hline
Supervox. Oracle perf.   &         & 79.57\%                                                                   & 87.76\%                        & 84.13\%                                \\ \hline
Full network   & 87.95\%   & 89.59\%                                                                   & 88.97\%                        & \textbf{89.91\%}                       \\
Reduction (/4) & 78.89\%   & 82.67\%                                                                   & 82.27\%                        & \textbf{83.31\%}                       \\
Reduction (/8) & 72.16\%   & 75.22\%                                                                   & 76.87\%                        & \textbf{78.90\%}                       \\ \bottomline
\end{tabular}
\end{table}
